Direct Construction of Optimal Z-Complementary Code Sets for all Possible Even Length by Using Pseudo-Boolean Functions

Z-complementary code set (ZCCS) are well known to be used in multicarrier code-division multiple access (MCCDMA) system to provide a interference free environment. Based on the existing literature, the direct construction of optimal ZCCSs are limited to its length. In this paper, we are interested in constructing optimal ZCCSs of all possible even lengths using Pseudo-Boolean functions. The maximum column sequence peakto-man envelop power ratio (PMEPR) of the proposed ZCCSs is upper-bounded by two, which may give an extra benefit in managing PMEPR in an ZCCS based MC-CDMA system, as well as the ability to handle a large number of users.

==> fjfjyhfjh.tex <==
Now we truncate the sequence $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  by reomoving  all the elements of the form  $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$  from $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$     if  atleast one of $i_{k}\geq p_{k}$ where $0\leq i_{k}\leq2^{s_k}-1$,  $1\leq k\leq l$ and $0\leq j\leq 2^{m}-1$. Therefore after the trancation we left with a squence $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  where, each elements of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is of the form  $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$\!\! where, $0\!\leq i_{k}\leq\! p_{k}\!-\!1$ , $0\!\leq\! j\!\leq\! 2^{m}\!-\!1$ and $1\leq\! k\!\leq\! l$. Clearly we can 
\newpage
~
 \begin{strip}
 \begin{equation}
    \begin{split}
        &\Psi^{i}_{Trun}(M^{\mathbf{v},r,d,\lambda,h})=\underbrace{(w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots, (w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}}\\
 &\Psi^{i}_{Trun}(M^{\mathbf{v},r,d,\lambda,h})=\underbrace{(w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots, (w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}}\\
    \end{split}
 \end{equation}
 \end{strip}
 and $j$ from $0$ to $2^{m}\!-\!1$. Hence the length of  $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is 
 $p_{1}p_{2}\hdots p_{k}2^{m}$.
 In this way we obtain the sequence $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$. Similarly by the same way 
 we obtain the sequence $\Psi_{Trun}(N^{\mathbf{v'},\mathbf{r},\lambda,h})$. We can partition the length of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ by $\prod_{i=1}^{l}p_{i}$ parenthesis where each parenthesis contains $2^{m}$ elements. Equation (10) represents the $i$-th parenthesis of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ and $\Psi_{Trun}(N^{\mathbf{v'},\mathbf{r},\lambda,h})$ where $i=i_{1}+\displaystyle\sum_{j=2}^{l}\prod_{b=1}^{j-1}p_{b}(i_{j})$, $0\leq i_{j}\leq p_{j}-1$ and $1\leq j \leq l$.

 \section{Proposed Construction of ZCCs}
\begin{theorem}
 Let $g:Z_{2}^m \rightarrow Z_{q}$ be a GBF as defined in \textit{Lemma} \textit{2}. Let $2\leq  p_i< 2^{s_i}$   and $\lambda=(\lambda_1,\lambda_2,\ldots,\lambda_l)$ where $1\leq i\leq l$ and $0\leq\lambda_{i}\leq p_{i}$. Then the set of codes
\begin{equation}
    \begin{split}
 \bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi^{*}_{Trun}}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}<p_{i}-1\bigg\},
    \end{split}
\end{equation}
forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$ if $h(\mathbf{v}')\!\in \{c,\frac{q}{2}+c\}$ $\forall \mathbf{v'}\in \{0,1\}^{n+1}$, where $c\in Z_{q}$.
\end{theorem}
\begin{IEEEproof}
From (10) it can be observed that the $i$-th  parenthesis of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ and $\Psi_{Trun}(N^{\mathbf{v'},\mathbf{r},\lambda,h})$ can be expressed as  $\omega_{p_1}^{\lambda_1 (i_1)}\omega_{p_2}^{\lambda_2 (i_2)}\ldots\omega_{p_l}^{\lambda_l (i_l)}\Psi(g^{\mathbf{v'},\mathbf{r},h})$ and\!\!\!\!  $\omega_{p_1}^{\lambda_1 (i_1)}\omega_{p_2}^{\lambda_2 (i_2)}\ldots\omega_{p_l}^{\lambda_l (i_l)}\Psi(s^{\mathbf{v'},\mathbf{r},h})$ respectively, where $i=i_{1}+\displaystyle\sum_{j=2}^{l}\prod_{b=1}^{j-1}p_{b}(i_{j})$, $0\leq i_{j}\leq p_{j}-1$ and $1\leq j \leq l$.
From (8), (10), \textit{Lemma} \textit{1} and \textit{Lemma} \textit{2} the ACCF between $\Psi_{Trun}(\Omega_{r}^{\lambda})$ and ${\Psi_{Trun}}(\Omega_{r'}^{\lambda'})$   for $\tau=0$ can be derived as,\\
\begin{equation}
    \begin{split}
        &\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}}(\Omega_{r'}^{\lambda '}))(0)\\
        &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)\\
        &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi}(g^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}\\
        &=\Theta(\Psi(G_r),\Psi(G_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}\\
        &=\begin{cases}
     p_{1}p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\\
     0         ,& r=r', \lambda\neq\lambda',\\
     0         ,& r\neq r',\lambda=\lambda',\\
     0         ,& r\neq r',\lambda\neq \lambda'.
    \end{cases}
    \end{split}
\end{equation}
Now, Using (8), (10), \textit{Lemma} \textit{1} and  the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ 
and ${\Psi_{Trun}}(\Omega_{t'}^{\lambda^{'}})$ for $0<|\tau|<2^m$ can be derived as,
\begin{equation}
    \begin{split}
        &\Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda^{'}}))(\tau)\\
        &=\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_i-1}\omega_{p_{i}}^{(\lambda_i-\lambda_i^{'})(\alpha)}\\
         &+\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau-2^m)\displaystyle\sum_{\alpha=0}^{p_{1}-2}\omega_{p_{1}}^{\lambda_1(\alpha+1)-\lambda_1^{'}\alpha}\\
        &\prod_{i=2}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_{i}}^{\lambda_i(\alpha)-\lambda_i'(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\displaystyle\sum_{j=1}^{l-2}\prod_{i=1}^{j}\omega_{p_{i}}^{\lambda_{i}(0)-\lambda^{'}_{i}(p_{i}-1)}\displaystyle\sum_{\alpha=0}^{p_{j+1}-2}\omega_{p_{j+1}}^{\lambda_{j+1}(\alpha+1)-\lambda^{'}_{j+1}(\alpha)}\prod_{k=j+2}^{l}\\
        &\displaystyle\sum_{\alpha=0}^{p_{k}-1}\omega_{p_{k}}^{\lambda_{p_{k}}(\alpha)-\lambda^{'}_{p_{k}}(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\prod_{i=1}^{l-1}w_{p_i}^{\lambda_i( 0)-\lambda_i^{'}(p_i-1)}\displaystyle\sum_{\alpha=0}^{p_{l}-2}\omega_{p_{l}}^{\lambda_{l}(\alpha+1)-\lambda^{'}_{l}\alpha}.
    \end{split}
\end{equation}
From \textit{Lemma} \textit{1}, we have, $\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)=0$, $\forall$ $|\tau| \in \{1,2^{m}-1\}$. Therefore, from the above we can say,
\begin{equation}
 \begin{split}
    \Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda '}))(\tau)=0, 0<|\tau|<2^m.
 \end{split}
\end{equation}
From (14) and (16) We have,
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t'}^{\lambda '}))(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
Similarly, it can be shown that
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi^{*}_{Trun}}(\Lambda_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r'}^{\lambda'})(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
From \textit{Lemma} \textit{1}, we have 
$\Theta(\Psi(G_r),\Psi^*(\bar{G}_{r}))(\tau)=0,~ |\tau|<2^m.$
Therefore, from \textit{Lemma} \textit{1}, (8), (10) the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ and ${\Psi_{Trun}^{*}}(\Lambda_{t^{'}}^{\lambda^{'}})$ for $\tau=0$ can be derived as,
\newpage
\begin{equation}
    \begin{split}
    &\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)\\
    &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}^{*}}(N^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)\\
&=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi^{*}}(s^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i+\lambda_i')\alpha}\\
&=\omega_{q}^{2c}\Theta(\Psi(G_r),\Psi^{*}(\bar{G}_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i+\lambda_i')\alpha}\\
&=0.
    \end{split}
\end{equation}
By the similar calculation as in  (15), we have
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(\tau)=0,\forall~ 0<|\tau|<2^{m}.
\end{equation}
Hence by (17), (18), (20) and (22) we  conclude the set
\begin{equation}
\begin{split}
    \bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi_{Trun}}^{*}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}\leq p_{i}-1\bigg\},
\end{split}
\end{equation}
 forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$.
\end{IEEEproof}
\begin{corollary}
Our construction gives optimal ZCCS of length of this form $(p_{1}p_{2}\hdots,p_{l})2^{m}$, where $p_{i}$'s are any prime numbers. From the fundamental theorem of arithmetic \cite{baker1984concise}   any number can be expressed as product of prime numbers therefore  the optimal ZCCS obtained by using our suggested construction gives all possible  length  of this form $n2^{m}$, where $n$ is any positive integer greater than $1$. If $m=1$ we get all possible  even length optimal ZCCS.
\end{corollary}
\begin{remark}
 For $l=1$, the proposed result in Theorem 1 reduces to $(p2^{n+1}, 2^m)$-$ZCCS_{2^{n+1}}^{p2^m}$ as in [10]. Therefore, the proposed construction is a generalization of [10]
\end{remark}
\begin{corollary}(\cite{sarkar2020direct} )
 Let us assume that $G(h)$ is path where the
edges have the identical weight of $\frac{q}{2}$. Then $h(\mathbf{v'})$ can be expressed as
$$h(v_{0},v_{1},\hdots,v_{n})=\frac{q}{2}\sum_{\alpha=0}^{n-1}v_{\pi(\alpha)}v_{\pi(\alpha+1)}+\sum_{\alpha=0}^{n}u_{\alpha}v_{\alpha}+u,$$
where $u,u_{0},u_1,\hdots u_{n}\in \mathbb{Z}_{q}$. From (8), it is clear
that the $i$-th column of $\psi(\Omega_{r}^{\lambda})$ is obtained by fixing $\mathbf{\bar{y}}$ at  $\mathbf{{i}}\!\!\!=\!\!\!(i_0,i_1,\hdots,i_{m},\hdots,i_{{m+\sum_{i=1}^{l}s_i}-1})$, in the  expression of $M^{\mathbf{v'},r,\lambda,h}$
where $(i_0,i_1,\hdots,i_{m},\hdots,i_{{m+\sum_{i=1}^{l}s_i}-1})$ is the binary representation of $i$.
Because the $i$-th column sequence of $\Psi(\Omega_t^\lambda)$ is derived from a GBF whose graph is a path over n+1 vertices, hence from \cite{paterson2000generalized} the $i$-th column sequence of $\Psi(\Omega_t^\lambda)$ is a q-ary Golay sequence. Thus each coloumn of $\Psi_{Trun}(\Omega_t^\lambda)$ is Golay sequence. Thus the PMPER of each coloumn $\Psi_{Trun}(\Omega_t^\lambda)$ is bounded by $2$. Similarly each coloumn of $\Psi^{*}_{Trun}(\Lambda_t^\lambda)$ is bounded by $2$.
\begin{remark}
 From (11), it can be observed that $w_{q}^{M_{r'}^{\mathbf{v'},\mathbf{r},h}}$ is a root of the
polynomial: $z^{\sigma}-1$, where $\sigma=lcm(p_{1},p_{2},\hdots,p_{l},q)$, denotes a positive
integer given by the least common multiple (lcm) of $p_{1},p_{2},\hdots,p_{l}$ and $q$. Therefore, the components of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ are given by the roots of the polynomial: $z^{\sigma}-1$.
\end{remark}
 \begin{example}
Let us assume that $q\!=\!2$, $p_1\!=\!3$, $p_2\!=\!2$, $p_3\!=\!2$ $m=3$, $n=1$ and $s_1=2$, $s_2=1$ and $s_3=1$. Let us take the GBF $f:\{0,1\}^2\rightarrow\mathbb{Z}_2$ as follows:
 $f=y_1y_2+y_0$, where $G(f\arrowvert_{y_0=0})$ and $G(f\arrowvert_{y_0=1})$ give a path with $y_1$ as one of the end vertices. Let $h:\{0,1\}^{2}\rightarrow Z_{2}$ defined by $h(v_{0},v_{1})=v_{0}v_{1}$ From (7) we have,
 \begin{equation}
  \begin{split}
  & M^\lambda=y_1y_2+y_0+\frac{2\lambda_1 }{3}(y_3+2y_4)+\lambda_2 y_5+\lambda_3 y_6,\\
  & N^\lambda=\bar{y}{_1}\bar{y}{_2}+\bar{y}{_0}+\frac{2\lambda_1 }{3}(y_3+2y_4)+\lambda_2 y_5+\lambda_3 y_6,
  \end{split}
 \end{equation}
 where $\lambda_1=0,1,2$, $\lambda_2=0,1$ and $\lambda_3=0,1$ From (8), we have
\begin{equation}
\begin{split}
 \Omega_r^\lambda&=\left\{M^\lambda+v_{0}v_{1}+v_0y_0+r_0y_0+v_{1}y_1:v_0,v_{1}\in\{0,1\}\right\},\\
 \Lambda_r^\lambda&=\left\{N^\lambda+v_{0}v_{1}+v_0\bar{y}_0+r_0\bar{y}_0+\bar{v}_{1}y_1:v_0,v_1\in\{0,1\}\right\},
 \end{split}
\end{equation}
where $(r_0)$ is the binary  representation of the integer $r$ and $0\leq r<2$. Therefore,
\begin{align*}
\begin{split}
    \Big\{\bar{\psi}(\Omega_{r}^{\lambda}),\bar{\psi}^{*}(\Lambda_{r}^{\lambda}):0\leq r\leq 1, 0\leq \lambda_1\leq 2,0\leq &\lambda_2\leq 1,\\&0\leq \lambda_3\leq 1\Big\},
\end{split}
\end{align*} forms an optimal $(48,8)$-ZCCS$_{4}^{96}$ and the maximum coloumn sequence PMPER is at most 2.
\end{example}
\end{corollary}
\begin{remark}
 Our proposed construction also have some advantage over [19].
 \begin{enumerate}
     \item In [19]  multivariable functions is used which is less feasible for hardware generation of sequences as their domains contain the domains of PBF as subset.
     \item Our construction  have more flexibility on the phases of sequences.
     \item Also in [19] the length of ZCCs is of the form $q^{m}$ where $m\geq 2$, $q\in Z^{+}$  which, may not produce all even lengths, for example 6.
 \end{enumerate}
 

\end{remark}
\begin{table}[!t]
\centering
\caption{Comparison of the Proposed Construction with \cite{sarkar2018optimal,das2020new,sarkar2020direct,wu2020z,sarkar2021pseudo,
shen2021new} }\label{ointa}
%\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Source           & Based On       &Parameters  &Coditions &Optimal     \\ \hline
\cite{sarkar2018optimal} &Direct        &$(2^{k+p+1},2^{m-p})-ZCCS_{2^{k+1}}^{2^m}$     & $k+p\leq m$   &yes                             \\ \hline
\cite{das2020new}&Indirect         &$(K,M)-ZCCS_{M}^{K}$     &$K,M\geq 2$ &yes                                 \\ \hline
\cite{sarkar2020direct}  &Direct         &$(2^{n+p},2^{m-p})-ZCCS_{2^n}^{2^m}$   &$p\leq m$
& yes \\ \hline
\cite{wu2020z}   &Direct          &$(2^{k+v},2^{m-v})-ZCCS_{2^{k}}^{2^m}$     &$v\leq m,k\leq m-v$ &yes                                      \\ \hline
\cite{sarkar2021pseudo} &Direct         &$(p2^{k+1},2^m)-ZCCS_{2^{k+1}}^{p2^m}$     &$m\geq 2$    &yes                                  \\ \hline
\cite{shen2021new} &Direct        &$(q^{v+1},q^{m-v})-ZCCS_{q}^{q^{m}}$ &$v\leq  m$         &yes                      \\ \hline
\cite{das2020new}&Indirect   &     $(K,M^{N+1})-ZCCS_{M}^{M^{N+1}P}$        &$K,M\geq 2$       &yes                           \\ \hline
\textit{Theorem 1} &Direct          &$(n2^{k+1},2^m)-ZCCS_{2^{k+1}}^{n2^m}$    &$ n\in \mathbf{Z}^{+},m\geq 2$            &yes                 \\ \hline
\end{tabular}}
\end{table}
\section{Conclusion}
In this work, we have proposed a direct construction of optimal ZCCSs for all possible even lengths using PBFs. The maximum column sequence PMEPR of the proposed  ZCCSs is upper-bounded by $2 $ which can be useful  in MC-CDMA systems to control high PMEPR problem. The proposed construction also provides more flexible parameter as compared to the existing PBFs based construction of optimal ZCCSs.
\bibliographystyle{IEEEtran}
\bibliography{Bibliography.bib}

==> fjgffhgfgh.tex <==
\begin{equation}
    \begin{split}
       &M^{\lambda}(\mathbf{{Y}})\!=\!g+\displaystyle\sum_{i=1}^{l}\frac{\lambda_{i}q}{p_{i}}(\displaystyle\sum_{k=0}^{s_{i}-1}2^{k}y_{m+{\sum_{j=0}^{i-1}s_{j}+k}})\\
        &M^{\lambda}(\mathbf{{Y}})\!=\!g+\displaystyle\sum_{i=1}^{l}\frac{\lambda_{i}q}{p_{i}}(\displaystyle\sum_{k=0}^{s_{i}-1}2^{k}y_{m+{\sum_{j=0}^{i-1}s_{j}+k}}) 
    \end{split}
\end{equation}
where each $y_{i}$'s are Boolean variable.
From above, it is clear that both $M^{\lambda}$ and $N^{\lambda}$ are PBF of variables $m+\sum_{i=1}^{l}s_i$. We chose $s_i$ in such a way that $p_i\leq 2^{s_i}-1$. If $p_i|q$ $\forall i$, then $M^{\lambda}$ and $N^{\lambda}$ reduces to GBFs.\\
Let $\!h\!:\!\{0,1\}^{n+1}\rightarrow Z_{q}$ be a $q$-ary function  and $\mathbf{r}=(r_0,r_1,\hdots, r_{n-1})$ be the binary representation of the integer $r$ where, $0\leq r<2^n$, and $\lambda=(\lambda_1,\lambda_2,\ldots, \lambda_l)$.
We define the set of PBFs as,
 \begin{equation}
     \begin{split}
       &\Omega_r^\lambda\!\!=\!\!\Big\{{M}^\lambda(\mathbf{Y})+h(\mathbf{v'})\!+\!
 \frac{q}{2}\Big((\mathbf{v}+\mathbf{r})\cdot {\mathbf{y}}
 \!+\!{v_{n}}y_{\gamma} \Big)\\
 &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~:\mathbf{v}\in \{0,1\}^n,v_{n}\in\{0,1\}\Big\},\\
 &\Lambda_r^\lambda\!\!=\!\!\Big\{{N}^\lambda(\mathbf{Y})+h(\mathbf{v'})\!+\!
 \frac{q}{2}\Big((\mathbf{v}+\mathbf{r})\cdot {\mathbf{\bar{y}}}
 \!+\!{\bar{v}_{n}}y_{\gamma} \Big)\\
 &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~:\mathbf{v}\in \{0,1\}^n,{v}_{n}\in\{0,1\}\Big\},
     \end{split}
 \end{equation}   
where, $\!\!\!\mathbf{v'}\!\!\!\!\!=\!\!\!\!\!(\mathbf{v},v_{n})\!\!\!\!\!=\!\!\!\!\!(v_{0},v_{1},\hdots,v_{n})$.\!\!\!
Let\! us assume that $g$ be the GBF as defined in \textit{Lemma} \textit{1}. Let $g^{\mathbf{v'},\mathbf{r},h}\!\!=\!\!g+h(\mathbf{v'})+\frac{q}{2}((\mathbf{v}+\mathbf{r})\cdot \mathbf{y}
 \!+v_{n}y_{\gamma})~ and ~ 
 s^{\mathbf{v'},\mathbf{r},h}\!\!=\!\!\tilde{g}+h(\mathbf{v'})+\frac{q}{2}((\mathbf{v}+\mathbf{r})\cdot \bar{\mathbf{y}}
 \!+\bar{v}_{n}y_{\gamma})$ in \textit{Lemma} \textit{1}. We also assume $M^{\mathbf{v'},\mathbf{r},\lambda,h}=M^\lambda+h(\mathbf{v'})\!\!+\!\frac{q}{2}((\mathbf{v}+\mathbf{r})\cdot \mathbf{y})
 \!+\!v_{n}y_{\gamma}$  and $N^{\mathbf{v'},\mathbf{r},\lambda,h}=N^\lambda+h(\mathbf{v'})\!+\!
 \frac{q}{2}((\mathbf{v}+\mathbf{r})\cdot \bar{\mathbf{y}}
 \!+\!\bar{v}_{n}y_{\gamma})$, in (8). As per our assumption, for any choice of $\mathbf{v'}\in \{0,1\}^{n+1}$ and $\mathbf{r}\in \{0,1\}^n$,
 the functions $g^{\mathbf{v'},\mathbf{r},h}$ and $s^{\mathbf{v'},\mathbf{r},h}$ are $\mathbb{Z}_q$-valued GBFs of $m$ variables. For any choice 
 of $\mathbf{v'}\in \{0,1\}^{n+1}$ and $\mathbf{r}\in \{0,1\}^n,$  $\lambda=(\lambda_1,\lambda_2,\hdots, \lambda_l)$ and $h$ the functions  
 $M^{\mathbf{v'},\mathbf{r},\lambda,h}$ and $N^{\mathbf{v'},\mathbf{r},\lambda,h}$ are PBFs of $m+\sum_{i=0}^{l}s_i$ variables.
We define $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$, the complex-valued sequence corresponding to $M^{\mathbf{v'},\mathbf{r},\lambda,h}$, as  $ \Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})=
 &(\omega^{M^{\mathbf{v'},\mathbf{r},\lambda,h}_0}_q, \omega^{M^{\mathbf{v'},\mathbf{r},\lambda,h}_1}_q,\hdots,\omega_q^{M^{\mathbf{v'},\mathbf{r},\lambda,h}_{2^{m+\sum_{i=0}^{l}s_i}-1}})$,

  where, $M^{\mathbf{v'},\mathbf{r},\lambda,h}_{r'}\!\!\!=\!\!\!M^{\mathbf{v'},\mathbf{r},\lambda,h}(r_0,r_1,\hdots,r_{m+\sum_{i=0}^{l}s_i-1})$, $0\!\leq\! r'\!<\!2^{m+\sum_{i=0}^{l}s_i}$
and  the binary representation of the integer $r'$ is  $(r_0,r_1,\hdots,r_{m+\sum_{i=0}^{l}s_i-1})$.  The $r'$-th component of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is given by, where,\!\!\! $(r_{0},r_{1},\hdots,r_{m-1})$\! is the binary representation of the integer $j$.
Since $M^{\mathbf{v'},\mathbf{r},\lambda,h}$ is a $m\!+\!\sum_{i=1}^{l}s_{i}$ variable PBF therefore  the length of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  is $2^{s_1}2^{s_2}\ldots2^{s_l}2^{m}$. Any element of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is of the form $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})}$,\! where $0\leq i_{k}\!\leq\!2^{s_{k}\!}-\!1$, $0\leq j\leq 2^{m}-1$ and $0\leq k\leq l$.
If $S=\{P_1,P_2,\hdots,P_e\}$ be collection of $e$ PBFs where each PBFs has same number of varible $a$
then 
    $\Psi(S)=\big[
\Psi(P_1),
\Psi(P_2),
\hdots,
\Psi(P_e)\big]^{T}_{2^{a}\times e}$.
\begin{remark}
 From (11), it can be observed that $w_{q}^{M_{r'}^{\mathbf{v'},\mathbf{r},h}}$ is a root of the
polynomial: $z^{\sigma}-1$, where $\sigma=lcm(p_{1},p_{2},\hdots,p_{l},q)$, denotes a positive
integer given by the least common multiple (lcm) of $p_{1},p_{2},\hdots,p_{l}$ and $q$. Therefore, the components of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ are given by the roots of the polynomial: $z^{\sigma}-1$.
\end{remark}

\newpage
~
 \begin{strip}
 \begin{equation}
    \begin{split}
        &\Psi^{i}_{Trun}(M^{\mathbf{v},r,d,\lambda,h})=\underbrace{(w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots, (w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}}\\
 &\Psi^{i}_{Trun}(M^{\mathbf{v},r,d,\lambda,h})=\underbrace{(w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots, (w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}}\\
    \end{split}
 \end{equation}
 \end{strip}
Now we truncate the sequence $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  by reomoving  all the elements of the form  $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$  from $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$     if  atleast one of $i_{k}\geq p_{k}$ where $0\leq i_{k}\leq2^{s_k}-1$ , $1\leq k\leq l$ and $0\leq j\leq 2^{m}-1$. Therefore after the trancation we left with a squence $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  where, each elements of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is of the form  $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$\!\! where, $0\!\leq i_{k}\leq\! p_{k}\!-\!1$ , $0\!\leq\! j\!\leq\! 2^{m}\!-\!1$ and $1\leq\! k\!\leq\! l$. Clearly we can make $p_{1}p_{2}\hdots p_{k}2^{m}$ number of the elements of these form $w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})}w_{q}^{s_{j}^{\mathbf{v'},\mathbf{r},h}}$   if we vary all the $i_{k}$'s from $0$ to $p_{k}\!-\!1$ and $j$ from $0$ to $2^{m}\!-\!1$. Hence the length of  $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is 
 $p_{1}p_{2}\hdots p_{k}2^{m}$.
 In this way we obtain the sequence $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$. Similarly by the same way we obtain the sequence $\Psi_{Trun}(N^{\mathbf{v'},\mathbf{r},\lambda,h})$. We can partition the length of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ by $\prod_{i=1}^{l}p_{i}$ parenthesis where each parenthesis contains $2^{m}$ elements. Equation (10) represents the $i$-th parenthesis of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ and $\Psi_{Trun}(N^{\mathbf{v'},\mathbf{r},\lambda,h})$ where $i=i_{1}+\displaystyle\sum_{j=2}^{l}\prod_{b=1}^{j-1}p_{b}(i_{j})$, $0\leq i_{j}\leq p_{j}-1$ and $1\leq j \leq l$.
 \section{Proposed Construction of ZCCs}
\begin{theorem}
 Let $g:Z_{2}^m \rightarrow Z_{q}$ be a GBF as defined in \textit{Lemma} \textit{2}. Let $2\leq  p_i< 2^{s_i}$   and $\lambda=(\lambda_1,\lambda_2,\ldots,\lambda_l)$ where $1\leq i\leq l$ and $0\leq\lambda_{i}\leq p_{i}$. Then the set of codes
\begin{equation}
    \begin{split}
 \bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi^{*}_{Trun}}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}<p_{i}-1\bigg\},
    \end{split}
\end{equation}
forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$ if $h(\mathbf{v}')\!\in \{c,\frac{q}{2}+c\}$ $\forall \mathbf{v'}\in \{0,1\}^{n+1}$, where $c\in Z_{q}$.
\end{theorem}
\begin{IEEEproof}
From (10) it can be observed that the $i$-th  parenthesis of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ and $\Psi_{Trun}(N^{\mathbf{v'},\mathbf{r},\lambda,h})$ can be expressed as  $\omega_{p_1}^{\lambda_1 (i_1)}\omega_{p_2}^{\lambda_2 (i_2)}\ldots\omega_{p_l}^{\lambda_l (i_l)}\Psi(g^{\mathbf{v'},\mathbf{r},h})$ and\!\!\!\!  $\omega_{p_1}^{\lambda_1 (i_1)}\omega_{p_2}^{\lambda_2 (i_2)}\ldots\omega_{p_l}^{\lambda_l (i_l)}\Psi(s^{\mathbf{v'},\mathbf{r},h})$ respectively, where $i=i_{1}+\displaystyle\sum_{j=2}^{l}\prod_{b=1}^{j-1}p_{b}(i_{j})$, $0\leq i_{j}\leq p_{j}-1$ and $1\leq j \leq l$.
From (8), (10), \textit{Lemma} \textit{1} and \textit{Lemma} \textit{2} the ACCF between $\Psi_{Trun}(\Omega_{r}^{\lambda})$ and ${\Psi_{Trun}}(\Omega_{r'}^{\lambda'})$   for $\tau=0$ can be derived as,\\
\begin{equation}
    \begin{split}
        &\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}}(\Omega_{r'}^{\lambda '}))(0)\\
        &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)\\
        &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi}(g^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}\\
        &=\Theta(\Psi(G_r),\Psi(G_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}\\
        &=\begin{cases}
     p_{1}p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\\
     0         ,& r=r', \lambda\neq\lambda',\\
     0         ,& r\neq r',\lambda=\lambda',\\
     0         ,& r\neq r',\lambda\neq \lambda'.
    \end{cases}
    \end{split}
\end{equation}
Now, Using (8), (10), \textit{Lemma} \textit{1} and  the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ 
and ${\Psi_{Trun}}(\Omega_{t'}^{\lambda^{'}})$ for $0<|\tau|<2^m$ can be derived as,
\begin{equation}
    \begin{split}
        &\Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda^{'}}))(\tau)\\
        &=\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_i-1}\omega_{p_{i}}^{(\lambda_i-\lambda_i^{'})(\alpha)}\\
         &+\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau-2^m)\displaystyle\sum_{\alpha=0}^{p_{1}-2}\omega_{p_{1}}^{\lambda_1(\alpha+1)-\lambda_1^{'}\alpha}\\
        &\prod_{i=2}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_{i}}^{\lambda_i(\alpha)-\lambda_i'(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\displaystyle\sum_{j=1}^{l-2}\prod_{i=1}^{j}\omega_{p_{i}}^{\lambda_{i}(0)-\lambda^{'}_{i}(p_{i}-1)}\displaystyle\sum_{\alpha=0}^{p_{j+1}-2}\omega_{p_{j+1}}^{\lambda_{j+1}(\alpha+1)-\lambda^{'}_{j+1}(\alpha)}\prod_{k=j+2}^{l}\\
        &\displaystyle\sum_{\alpha=0}^{p_{k}-1}\omega_{p_{k}}^{\lambda_{p_{k}}(\alpha)-\lambda^{'}_{p_{k}}(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\prod_{i=1}^{l-1}w_{p_i}^{\lambda_i( 0)-\lambda_i^{'}(p_i-1)}\displaystyle\sum_{\alpha=0}^{p_{l}-2}\omega_{p_{l}}^{\lambda_{l}(\alpha+1)-\lambda^{'}_{l}\alpha}.
    \end{split}
\end{equation}
From \textit{Lemma} \textit{1}, we have, $\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)=0$, $\forall$ $|\tau| \in \{1,2^{m}-1\}$. Therefore, from the above we can say,
\begin{equation}
 \begin{split}
    \Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda '}))(\tau)=0, 0<|\tau|<2^m.
 \end{split}
\end{equation}
From (14) and (16) We have,
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t'}^{\lambda '}))(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
Similarly, it can be shown that
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi^{*}_{Trun}}(\Lambda_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r'}^{\lambda'})(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
From \textit{Lemma} \textit{1}, we have 
\begin{equation}
     \Theta(\Psi(G_r),\Psi^*(\bar{G}_{r}))(\tau)=0,~ |\tau|<2^m.
\end{equation}
From \textit{Lemma} \textit{1}, (8), (10) the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ and ${\Psi_{Trun}^{*}}(\Lambda_{t^{'}}^{\lambda^{'}})$ for $\tau=0$ can be derived as,
\begin{equation}
    \begin{split}
    &\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)\\
    &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}^{*}}(N^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)\\
&=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi^{*}}(s^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i+\lambda_i')\alpha}\\
&=\omega_{q}^{2c}\Theta(\Psi(G_r),\Psi^{*}(\bar{G}_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i+\lambda_i')\alpha},
    \end{split}
\end{equation}
from \textit{Lemma} \textit{1}, we have $\Theta(\Psi(G_r),\Psi^{*}(\bar{G}_{r^{'}}))(0)=0.$\\
Therefore,
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)=0.
\end{equation}
By the similar calculation as in  (15), we have
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(\tau)=0,\forall~ 0<|\tau|<2^{m}.
\end{equation}
Hence by (17), (18), (20) and (22) we  conclude the set
\begin{equation}
\begin{split}
    \bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi_{Trun}}^{*}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}\leq p_{i}-1\bigg\},
\end{split}
\end{equation}
 forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$.
\end{IEEEproof}
\begin{corollary}
Our construction gives optimal ZCCS of length of this form $(p_{1}p_{2}\hdots,p_{l})2^{m}$, where $p_{i}$'s are any prime numbers. From the fundamental theorem of arithmetic \cite{baker1984concise}   any number can be expressed as product of prime numbers therefore  the optimal ZCCS obtained by using our suggested construction gives all possible  length  of this form $n2^{m}$, where $n$ is any positive integer greater than $1$. If $m=1$ we get all possible  even length optimal ZCCS.
\end{corollary}
\begin{remark}
 For $l=1$, the proposed result in Theorem 1 reduces to $(p2^{n+1}, 2^m)$-$ZCCS_{2^{n+1}}^{p2^m}$ as in [10]. Therefore, the proposed construction is a generalization of [10]
\end{remark}
\begin{corollary}(\cite{sarkar2020direct} )
 Let us assume that $G(h)$ is path where the
edges have the identical weight of $\frac{q}{2}$. Then $h(\mathbf{v'})$ can be expressed as
$$h(v_{0},v_{1},\hdots,v_{n})=\frac{q}{2}\sum_{\alpha=0}^{n-1}v_{\pi(\alpha)}v_{\pi(\alpha+1)}+\sum_{\alpha=0}^{n}u_{\alpha}v_{\alpha}+u,$$
where $u,u_{0},u_1,\hdots u_{n}\in \mathbb{Z}_{q}$. From (8), it is clear
that the $i$-th column of $\psi(\Omega_{r}^{\lambda})$ is obtained by fixing $\mathbf{\bar{y}}$ at  $\mathbf{{i}}\!\!\!=\!\!\!(i_0,i_1,\hdots,i_{m},\hdots,i_{{m+\sum_{i=1}^{l}s_i}-1})$, in the  expression of $M^{\mathbf{v'},r,\lambda,h}$
where $(i_0,i_1,\hdots,i_{m},\hdots,i_{{m+\sum_{i=1}^{l}s_i}-1})$ is the binary representation of $i$.
Because the $i$-th column sequence of $\Psi(\Omega_t^\lambda)$ is derived from a GBF whose graph is a path over n+1 vertices, hence from \cite{paterson2000generalized} the $i$-th column sequence of $\Psi(\Omega_t^\lambda)$ is a q-ary Golay sequence. Thus each coloumn of $\Psi_{Trun}(\Omega_t^\lambda)$ is Golay sequence. Thus the PMPER of each coloumn $\Psi_{Trun}(\Omega_t^\lambda)$ is bounded by $2$. Similarly each coloumn of $\Psi^{*}_{Trun}(\Lambda_t^\lambda)$ is bounded by $2$.
 \begin{example}
Let us assume that $q\!=\!2$, $p_1\!=\!3$, $p_2\!=\!2$, $p_3\!=\!2$ $m=3$, $n=1$ and $s_1=2$, $s_2=1$ and $s_3=1$. Let us take the GBF $f:\{0,1\}^2\rightarrow\mathbb{Z}_2$ as follows:
 $f=y_1y_2+y_0$, where $G(f\arrowvert_{y_0=0})$ and $G(f\arrowvert_{y_0=1})$ give a path with $y_1$ as one of the end vertices. Let $h:\{0,1\}^{2}\rightarrow Z_{2}$ defined by $h(v_{0},v_{1})=v_{0}v_{1}$. From (8) we have 
\begin{equation}
\begin{split}
 \Omega_r^\lambda&=\left\{M^\lambda+v_{0}v_{1}+v_0y_0+r_0y_0+v_{1}y_1:v_0,v_{1}\in\{0,1\}\right\},\\
 \Lambda_r^\lambda&=\left\{N^\lambda+v_{0}v_{1}+v_0\bar{y}_0+r_0\bar{y}_0+\bar{v}_{1}y_1:v_0,v_1\in\{0,1\}\right\},
 \end{split}
\end{equation}
where $(r_0)$ is the binary  representation of the integer $r$ and $0\leq r<2$. Therefore,
\begin{align*}
\begin{split}
    \Big\{\bar{\psi}(\Omega_{r}^{\lambda}),\bar{\psi}^{*}(\Lambda_{r}^{\lambda}):0\leq r\leq 1, 0\leq \lambda_1\leq 2,0\leq &\lambda_2\leq 1,\\&0\leq \lambda_3\leq 1\Big\},
\end{split}
\end{align*} forms an optimal $(48,8)$-ZCCS$_{4}^{96}$ and the maximum coloumn sequence PMPER is at most 2.
\end{example}
\end{corollary}
\begin{table}[!t]
\centering
\caption{Comparison of the Proposed Construction with \cite{sarkar2018optimal,das2020new,sarkar2020direct,wu2020z,sarkar2021pseudo,
shen2021new} }\label{ointa}
%\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Source           & Based On       &Parameters  &Coditions &Optimal     \\ \hline
\cite{sarkar2018optimal} &Direct        &$(2^{k+p+1},2^{m-p})-ZCCS_{2^{k+1}}^{2^m}$     & $k+p\leq m$   &yes                             \\ \hline
\cite{das2020new}&Indirect         &$(K,M)-ZCCS_{M}^{K}$     &$K,M\geq 2$ &yes                                 \\ \hline
\cite{sarkar2020direct}  &Direct         &$(2^{n+p},2^{m-p})-ZCCS_{2^n}^{2^m}$   &$p\leq m$
& yes \\ \hline
\cite{wu2020z}   &Direct          &$(2^{k+v},2^{m-v})-ZCCS_{2^{k}}^{2^m}$     &$v\leq m,k\leq m-v$ &yes                                      \\ \hline
\cite{sarkar2021pseudo} &Direct         &$(p2^{k+1},2^m)-ZCCS_{2^{k+1}}^{p2^m}$     &$m\geq 2$    &yes                                  \\ \hline
\cite{shen2021new} &Direct        &$(q^{v+1},q^{m-v})-ZCCS_{q}^{q^{m}}$ &$v\leq  m$         &yes                      \\ \hline
\cite{das2020new}&Indirect   &     $(K,M^{N+1})-ZCCS_{M}^{M^{N+1}P}$        &$K,M\geq 2$       &yes                           \\ \hline
\textit{Theorem 1} &Direct          &$(n2^{k+1},2^m)-ZCCS_{2^{k+1}}^{n2^m}$    &$ n\in \mathbf{Z}^{+},m\geq 2$            &yes                 \\ \hline
\end{tabular}}
\end{table}
\section{Conclusion}
In this work, we have proposed a direct construction of optimal ZCCSs for all possible even lengths using PBFs. The maximum column sequence PMEPR of the proposed  ZCCSs is upper-bounded by $2 $ which can be useful  in MC-CDMA systems to control high PMEPR problem. The proposed construction also provides more flexible parameter as compared to the existing PBFs based construction of optimal ZCCSs.

==> hjfjhfjhfhj.tex <==
Similarly, it can be shown that
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi^{*}_{Trun}}(\Lambda_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r'}^{\lambda'})(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
  From \textit{Lemma} \textit{1}, we have 
\begin{equation}
     \Theta(\Psi(G_r),\Psi^*(\bar{G}_{r}))(\tau)=0,~ |\tau|<2^m.
\end{equation}
From \textit{Lemma} \textit{1}, (8), (10) the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ and ${\Psi_{Trun}^{*}}(\Lambda_{t^{'}}^{\lambda^{'}})$ for $\tau=0$ can be derived as,
\begin{equation}
    \begin{split}
    &\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)\\
    &=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}^{*}}(N^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)\\
&=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi^{*}}(s^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i+\lambda_i')\alpha}\\
&=\omega_{q}^{2c}\Theta(\Psi(G_r),\Psi^{*}(\bar{G}_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i+\lambda_i')\alpha},
    \end{split}
\end{equation}
from \textit{Lemma} \textit{1}, we have $\Theta(\Psi(G_r),\Psi^{*}(\bar{G}_{r^{'}}))(0)=0.$\\
Therefore,
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)=0.
\end{equation}
By the similar calculation as in  (15), we have
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(\tau)=0,\forall~ 0<|\tau|<2^{m}.
\end{equation}
Hence by (17), (18), (20) and (22) we  conclude the set
\begin{equation}
\begin{split}
    \bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi_{Trun}}^{*}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}\leq p_{i}-1\bigg\},
\end{split}
\end{equation}
 forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$.
\end{IEEEproof}
\begin{corollary}
Our construction gives optimal ZCCS of length of this form $(p_{1}p_{2}\hdots,p_{l})2^{m}$, where $p_{i}$'s are any prime numbers. From the fundamental theorem of arithmetic \cite{baker1984concise}   any number can be expressed as product of prime numbers therefore  the optimal ZCCS obtained by using our suggested construction gives all possible  length  of this form $n2^{m}$, where $n$ is any positive integer greater than $1$. If $m=1$ we get all possible  even length optimal ZCCS.
\end{corollary}
\begin{remark}
 For $l=1$, the proposed result in Theorem 1 reduces to $(p2^{n+1}, 2^m)$-$ZCCS_{2^{n+1}}^{p2^m}$ as in [10]. Therefore, the proposed construction is a generalization of [10]
\end{remark}
\begin{corollary}(\cite{sarkar2020direct} )
 Let us assume that $G(h)$ is path where the
edges have the identical weight of $\frac{q}{2}$. Then $h(\mathbf{v'})$ can be expressed as
$$h(v_{0},v_{1},\hdots,v_{n})=\frac{q}{2}\sum_{\alpha=0}^{n-1}v_{\pi(\alpha)}v_{\pi(\alpha+1)}+\sum_{\alpha=0}^{n}u_{\alpha}v_{\alpha}+u,$$
where $u,u_{0},u_1,\hdots u_{n}\in \mathbb{Z}_{q}$. From (8), it is clear
that the $i$-th column of $\psi(\Omega_{r}^{\lambda})$ is obtained by fixing $\mathbf{\bar{y}}$ at  $\mathbf{{i}}\!\!\!=\!\!\!(i_0,i_1,\hdots,i_{m},\hdots,i_{{m+\sum_{i=1}^{l}s_i}-1})$, in the  expression of $M^{\mathbf{v'},r,\lambda,h}$
where $(i_0,i_1,\hdots,i_{m},\hdots,i_{{m+\sum_{i=1}^{l}s_i}-1})$ is the binary representation of $i$.
Because the $i$-th column sequence of $\Psi(\Omega_t^\lambda)$ is derived from a GBF whose graph is a path over n+1 vertices, hence from \cite{paterson2000generalized} the $i$-th column sequence of $\Psi(\Omega_t^\lambda)$ is a q-ary Golay sequence. Thus each coloumn of $\Psi_{Trun}(\Omega_t^\lambda)$ is Golay sequence. Thus the PMPER of each coloumn $\Psi_{Trun}(\Omega_t^\lambda)$ is bounded by $2$. Similarly each coloumn of $\Psi^{*}_{Trun}(\Lambda_t^\lambda)$ is bounded by $2$.
\begin{example}
Let us assume that $q\!=\!2$, $p_1\!=\!3$, $p_2\!=\!2$, $p_3\!=\!2$ $m=3$, $n=1$ and $s_1=2$, $s_2=1$ and $s_3=1$. Let us take the GBF $f:\{0,1\}^2\rightarrow\mathbb{Z}_2$ as follows:
 $f=y_1y_2+y_0$, where $G(f\arrowvert_{y_0=0})$ and $G(f\arrowvert_{y_0=1})$ give a path with $y_1$ as one of the end vertices. Let $h:\{0,1\}^{2}\rightarrow Z_{2}$ defined by $h(v_{0},v_{1})=v_{0}v_{1}$ From (7) we have,
 \begin{equation}
  \begin{split}
  & M^\lambda=y_1y_2+y_0+\frac{2\lambda_1 }{3}(y_3+2y_4)+\lambda_2 y_5+\lambda_3 y_6,\\
  & N^\lambda=\bar{y}{_1}\bar{y}{_2}+\bar{y}{_0}+\frac{2\lambda_1 }{3}(y_3+2y_4)+\lambda_2 y_5+\lambda_3 y_6,
  \end{split}
 \end{equation}
 where $\lambda_1=0,1,2$, $\lambda_2=0,1$ and $\lambda_3=0,1$ From (8), we have
\begin{equation}
\begin{split}
 \Omega_r^\lambda&=\left\{M^\lambda+v_{0}v_{1}+v_0y_0+r_0y_0+v_{1}y_1:v_0,v_{1}\in\{0,1\}\right\},\\
 \Lambda_r^\lambda&=\left\{N^\lambda+v_{0}v_{1}+v_0\bar{y}_0+r_0\bar{y}_0+\bar{v}_{1}y_1:v_0,v_1\in\{0,1\}\right\},
 \end{split}
\end{equation}
where $(r_0)$ is the binary  representation of the integer $r$ and $0\leq r<2$. Therefore,
\begin{align*}
\begin{split}
    \Big\{\bar{\psi}(\Omega_{r}^{\lambda}),\bar{\psi}^{*}(\Lambda_{r}^{\lambda}):0\leq r\leq 1, 0\leq \lambda_1\leq 2,0\leq &\lambda_2\leq 1,\\&0\leq \lambda_3\leq 1\Big\},
\end{split}
\end{align*} forms an optimal $(48,8)$-ZCCS$_{4}^{96}$ and the maximum coloumn sequence PMPER is at most 2.
\end{example}
\end{corollary}
\begin{table}[!t]
\centering
\caption{Comparison of the Proposed Construction with \cite{sarkar2018optimal,das2020new,sarkar2020direct,wu2020z,sarkar2021pseudo,
shen2021new} }\label{ointa}
%\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Source           & Based On       &Parameters  &Coditions &Optimal     \\ \hline
\cite{sarkar2018optimal} &Direct        &$(2^{k+p+1},2^{m-p})-ZCCS_{2^{k+1}}^{2^m}$     & $k+p\leq m$   &yes                             \\ \hline
\cite{das2020new}&Indirect         &$(K,M)-ZCCS_{M}^{K}$     &$K,M\geq 2$ &yes                                 \\ \hline
\cite{sarkar2020direct}  &Direct         &$(2^{n+p},2^{m-p})-ZCCS_{2^n}^{2^m}$   &$p\leq m$
& yes \\ \hline
\cite{wu2020z}   &Direct          &$(2^{k+v},2^{m-v})-ZCCS_{2^{k}}^{2^m}$     &$v\leq m,k\leq m-v$ &yes                                      \\ \hline
\cite{sarkar2021pseudo} &Direct         &$(p2^{k+1},2^m)-ZCCS_{2^{k+1}}^{p2^m}$     &$m\geq 2$    &yes                                  \\ \hline
\cite{shen2021new} &Direct        &$(q^{v+1},q^{m-v})-ZCCS_{q}^{q^{m}}$ &$v\leq  m$         &yes                      \\ \hline
\cite{das2020new}&Indirect   &     $(K,M^{N+1})-ZCCS_{M}^{M^{N+1}P}$        &$K,M\geq 2$       &yes                           \\ \hline
\textit{Theorem 1} &Direct          &$(n2^{k+1},2^m)-ZCCS_{2^{k+1}}^{n2^m}$    &$ n\in \mathbf{Z}^{+},m\geq 2$            &yes                 \\ \hline
\end{tabular}}
\end{table}
\section{Conclusion}
In this work, we have proposed a direct construction of optimal ZCCSs for all possible even lengths using PBFs. The maximum column sequence PMEPR of the proposed  ZCCSs is upper-bounded by $2 $ which can be useful  in MC-CDMA systems to control high PMEPR problem. The proposed construction also provides more flexible parameter as compared to the existing PBFs based construction of optimal ZCCSs.







\begin{equation}
             =\begin{cases}
     p_{1}p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\\
     0         ,& r=r', \lambda\neq\lambda',\\
     0         ,& r\neq r',\lambda=\lambda',\\
     0         ,& r\neq r',\lambda\neq \lambda'.~~~~~~~~~~~~
     \end{cases}
        \end{equation}
        Now, Using (8), (10), \textit{Lemma} \textit{1} and  the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ 
and ${\Psi_{Trun}}(\Omega_{t'}^{\lambda^{'}})$ for $0<|\tau|<2^m$ can be derived as,
\begin{equation}
    \begin{split}
        &\Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda^{'}}))(\tau)\\
        &=\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_i-1}\omega_{p_{i}}^{(\lambda_i-\lambda_i^{'})(\alpha)}\\
         &+\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau-2^m)\displaystyle\sum_{\alpha=0}^{p_{1}-2}\omega_{p_{1}}^{\lambda_1(\alpha+1)-\lambda_1^{'}\alpha}\\
        &\prod_{i=2}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_{i}}^{\lambda_i(\alpha)-\lambda_i'(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\displaystyle\sum_{j=1}^{l-2}\prod_{i=1}^{j}\omega_{p_{i}}^{\lambda_{i}(0)-\lambda^{'}_{i}(p_{i}-1)}\displaystyle\sum_{\alpha=0}^{p_{j+1}-2}\omega_{p_{j+1}}^{\lambda_{j+1}(\alpha+1)-\lambda^{'}_{j+1}(\alpha)}\prod_{k=j+2}^{l}\\
        &\displaystyle\sum_{\alpha=0}^{p_{k}-1}\omega_{p_{k}}^{\lambda_{p_{k}}(\alpha)-\lambda^{'}_{p_{k}}(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\prod_{i=1}^{l-1}w_{p_i}^{\lambda_i( 0)-\lambda_i^{'}(p_i-1)}\displaystyle\sum_{\alpha=0}^{p_{l}-2}\omega_{p_{l}}^{\lambda_{l}(\alpha+1)-\lambda^{'}_{l}\alpha}.
    \end{split}
\end{equation}
From \textit{Lemma} \textit{1}, we have, $\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)=0$, $\forall$ $|\tau| \in \{1,2^{m}-1\}$. Therefore, from the above we can say,
\begin{equation}
 \begin{split}
    \Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda '}))(\tau)=0, 0<|\tau|<2^m.
 \end{split}
\end{equation}
From (14) and (16) We have,
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t'}^{\lambda '}))(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}





\begin{lemma}({\cite{vaidyanathan2014ramanujan}} )\label{L3} Let $t$ and $t'$ be two non-negative integers, where $0\leq t\neq t'<p_{i}$, $p_{i}$ is a prime number as defined in section-II. 
 Then 
 $\displaystyle\sum_{j=0}^{p_{i}-1}\omega_{p_{i}}^{(t-t')j}=0.$
\end{lemma}





\begin{remark}
 From (11), it can be observed that $w_{q}^{M_{r'}^{\mathbf{v'},\mathbf{r},h}}$ is a root of the
polynomial: $z^{\sigma}-1$, where $\sigma=lcm(p_{1},p_{2},\hdots,p_{l},q)$, denotes a positive
integer given by the least common multiple (lcm) of $p_{1},p_{2},\hdots,p_{l}$ and $q$. Therefore, the components of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ are given by the roots of the polynomial: $z^{\sigma}-1$.
\end{remark}

==> new2.tex <==
\begin{equation}\label{wvvd}
 \begin{split}
&w_{q}^{M_{r'}^{\mathbf{v}',\mathbf{r},h}}=\omega_q^{{g}^{\mathbf{v'},\mathbf{r},h}(r_0,r_1,\hdots, r_{m-1})}\omega_{p_1}^{\lambda_1\sum_{i=0}^{i=s_{1}-1}2^{i}r_{m+i}}\\&\omega_{p_2}^{\lambda_2\sum_{i=0}^{i=s_{2}-1}2^{i}r_{m+s_{1}+i}}\ldots\omega_{p_l}^{\lambda_l\sum_{i=0}^{i=s_{l}-1}2^{i}r_{m+\sum_{j=1}^{l-1}s_{j}+i}}\\&=\omega_q^{{g}_{j}^{\mathbf{v'},\mathbf{r},h}}\omega_{p_1}^{\lambda_1(i_{1})}\omega_{p_2}^{\lambda_2(i_{2})}\ldots\omega_{p_l}^{\lambda_l(i_{l})},\\
 \end{split}
\end{equation}

where,\!\!\! $(r_{0},r_{1},\hdots,r_{m-1})$\! is the binary representation of the integer $j$.
Since $M^{\mathbf{v'},\mathbf{r},\lambda,h}$ is a $m\!+\!\sum_{i=1}^{l}s_{i}$ variable PBF therefore  the length of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  is $2^{s_1}2^{s_2}\ldots2^{s_l}2^{m}$. Any element of $\Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is of the form $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})}$,\! where $0\leq i_{k}\!\leq\!2^{s_{k}\!}-\!1$, $0\leq j\leq 2^{m}-1$ and $0\leq k\leq l$.
If $S=\{P_1,P_2,\hdots,P_e\}$ be collection of $e$ PBFs where each PBFs has same number of varible $a$
then 
    $\Psi(S)=\big[
\Psi(P_1),
\Psi(P_2),
\hdots,
\Psi(P_e)\big]^{T}_{2^{a}\times e}$.
\begin{lemma}({\cite{vaidyanathan2014ramanujan}} )\label{L3} Let $t$ and $t'$ be two non-negative integers, where $0\leq t\neq t'<p_{i}$, $p_{i}$ is a prime number as defined in section-II. 
 Then 
 $\displaystyle\sum_{j=0}^{p_{i}-1}\omega_{p_{i}}^{(t-t')j}=0.$
\end{lemma}

==> new5.tex <==

\newpage
 ~
 \begin{strip}
 \begin{equation}
     \begin{split}
          &~~~\Psi_{Trun}(M^{\mathbf{v},r,d,\lambda,h})\\
        &=\underbrace{(w_{p_1}^{\lambda_{1}(0)}w_{p_2}^{\lambda_{2}(0)}\hdots w_{p_l}^{\lambda_{l}(0)})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots,( w_{p_1}^{\lambda_{1}(0)}
 {w_{p_2}^{\lambda_{2}(0)}\hdots  w_{p_l}^{\lambda_{l}(0)})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}}}\\
 &~~~~\underbrace{(w_{p_1}^{\lambda_{1}(1)}w_{p_2}^{\lambda_{2}(0)}\ldots w_{p_l}^{\lambda_{l}(0)})w_{q}^{g_{0}^{\mathbf{v},t,d,h}},
\hdots (w_{p_1}^{\lambda_{1}(1)}w_{p_2}^{\lambda_{2}(0)}\ldots w_{p_l}^{\lambda_{l}(0)})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}},\hdots,\\
&~~~\underbrace{(w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots, (w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}},\hdots\\
&~~~\underbrace{(w_{p_1}^{\lambda_{1}(p_{1}-1)}w_{p_2}^{\lambda_{2}(p_{2}-1)}\hdots w_{p_l}^{\lambda_{l}(p_{l}-1)})w_{q}^{g_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots (w_{p_1}^{\lambda_{1}(p_{1}-1)}
w_{p_2}^{\lambda_{2}(p_{2}-1)}\hdots w_{p_l}^{\lambda_{l}(p_{l}-1)})w_{q}^{g_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}},\\
\vspace{0.2cm}
 &~~~\Psi_{Trun}(N^{\mathbf{v},r,d,\lambda,h})\\
        &=\underbrace{(w_{p_1}^{\lambda_{1}(0)}w_{p_2}^{\lambda_{2}(0)}\hdots w_{p_l}^{\lambda_{l}(0)})w_{q}^{s_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots,( w_{p_1}^{\lambda_{1}(0)}
 {w_{p_2}^{\lambda_{2}(0)}\hdots  w_{p_l}^{\lambda_{l}(0)})w_{q}^{s_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}}}\\
 &~~~~\underbrace{(w_{p_1}^{\lambda_{1}(1)}w_{p_2}^{\lambda_{2}(0)}\ldots w_{p_l}^{\lambda_{l}(0)})w_{q}^{s_{0}^{\mathbf{v},t,d,h}},
\hdots (w_{p_1}^{\lambda_{1}(1)}w_{p_2}^{\lambda_{2}(0)}\ldots w_{p_l}^{\lambda_{l}(0)})w_{q}^{s_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}},\hdots,\\
&~~~\underbrace{(w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{s_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots, (w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots w_{p_l}^{\lambda_{l}(i_{l})})w_{q}^{s_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}},\hdots\\
&~~~\underbrace{(w_{p_1}^{\lambda_{1}(p_{1}-1)}w_{p_2}^{\lambda_{2}(p_{2}-1)}\hdots w_{p_l}^{\lambda_{l}(p_{l}-1)})w_{q}^{s_{0}^{\mathbf{v},\mathbf{r},d,h}},\hdots (w_{p_1}^{\lambda_{1}(p_{1}-1)}
w_{p_2}^{\lambda_{2}(p_{2}-1)}\hdots w_{p_l}^{\lambda_{l}(p_{l}-1)})w_{q}^{s_{2^{m}-1}^{\mathbf{v},\mathbf{r},d,h}}},
     \end{split}
 \end{equation}
 \end{strip}
 \begin{equation}\label{wvvd}
 \begin{split}
&w_{q}^{M_{r'}^{v,r,d,h}}\\&=\omega_q^{{g}^{\mathbf{v},\mathbf{r},d,h}(r_0,r_1,\hdots, r_{m-1})}\omega_{p_1}^{\lambda_1\sum_{i=0}^{i=s_{1}-1}2^{i}r_{m+i}}\\&\omega_{p_2}^{\lambda_2\sum_{i=0}^{i=s_{2}-1}2^{i}r_{m+s_{1}+i}}\ldots\omega_{p_l}^{\lambda_l\sum_{i=0}^{i=s_{l}-1}2^{i}r_{m+\sum_{j=1}^{l-1}s_{j}+i}}\\&=\omega_q^{{g}_{j}^{\mathbf{v},\mathbf{r},d,h}}\omega_{p_1}^{\lambda_1(i_{1})}\omega_{p_2}^{\lambda_2(i_{2})}\ldots\omega_{p_l}^{\lambda_l(i_{l})}\\
 \end{split}
\end{equation}
where $(r_{0},r_{1},\hdots,r_{m-1})$ is the binary representation of the integer $j$.
Since $M^{\mathbf{v},r,d,\lambda,h}$ is a $m\!+\!\sum_{i=1}^{l}s_{i}$ variable PBF therefore  the length of $\Psi(M^{\mathbf{v},r,d,\lambda,h})$  is $2^{s_1}2^{s_2}\ldots2^{s_l}2^{m}$. Any element of $\Psi(M^{\mathbf{v},r,d,\lambda,h})$ is of the form $w_{q}^{g_{j}^{\mathbf{v},\mathbf{r},d,h}}w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})}$,\! where $0\leq i_{k}\!\leq\!2^{s_{k}\!}-\!1$, $0\leq j\leq 2^{m}-1$ and $0\leq k\leq l$.\\
If $S=\{P_1,P_2,\hdots,P_e\}$ be collection of $e$ PBFs where each PBFs has same number of varible $f$
then \begin{equation}
    \Psi(S)=\big[
\Psi(P_1),
\Psi(P_2),
\hdots,
\Psi(P_e)\big]^{T}_{2^{f}\times e}
\end{equation}
Now we truncate the sequence as follows we reomove  all the elements of the form  $w_{q}^{g_{j}^{\mathbf{v},\mathbf{r},d,h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$  from $\Psi(M^{\mathbf{v},r,d,\lambda,h})$     if  atleast one of $i_{k}\geq p_{k}$ where $0\leq i_{k}\leq2^{s_k}-1$ , $1\leq k\leq l$ and $0\leq j\leq 2^{m}-1$. Therefore after the trancation we left with a squence $\Psi_{Trun}(M^{\mathbf{v},r,d,\lambda,h})$ (14) where each elements of $\Psi_{Trun}(M^{\mathbf{v},r,d,\lambda,h})$ is of the form  $w_{q}^{g_{j}^{\mathbf{v},\mathbf{r},d,h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$, $0\!\leq i_{k}\leq\! p_{k}\!-\!1$ , $0\!\leq\! j\!\leq\! 2^{m}\!-\!1$ and $1\leq\! k\!\leq\! l$. Clearly we can make $p_{1}p_{2}\hdots p_{k}2^{m}$ number of the elements of the form $w_{p_1}^{\lambda_{1}(i_{1})}w_{p_2}^{\lambda_{2}(i_{2})}\hdots
w_{p_l}^{\lambda_{l}(i_{l})}w_{q}^{s_{j}^{\mathbf{v},\mathbf{r},d,h}}$   if we vary all the $i_{k}$'s from $0$ to $p_{k}\!-\!1$ and $j$ from $0$ to $2^{m}\!-\!1$. Hence the length of  $\Psi_{Trun}(M^{\mathbf{v},r,d,\lambda,h})$ is 
 $p_{1}p_{2}\hdots p_{k}2^{m}$.
 In this way we obtain the sequence $\Psi_{Trun}(M^{\mathbf{v},r,d,\lambda,h})$ as defined in (14). Similarly by the same way we obtain the sequence $\Psi_{Trun}(N^{\mathbf{v},r,d,\lambda,h})$ (15). Equation (14) and (15) contains $p_{1}p_{2}\hdots p_{l}$ parenthesis and each parenthesis has a sequence of length length $2^{m}$.
 \section{Proposed Construction of ZCCs}
 \begin{lemma}({\cite{vaidyanathan2014ramanujan}} )\label{L3} Let $t$ and $t'$ be two non-negative integers, where $0\leq t\neq t'<p_{i}$, $p_{i}$ is a prime number as defined in Section-II. 
 Then 
 $\displaystyle\sum_{j=0}^{p_{i}-1}\omega_{p_{i}}^{(t-t')j}=0.$
\end{lemma}
\begin{theorem}
 Let $g:Z_{2}^m \rightarrow Z_{q}$ be a GBF as defined in \textit{Lemma} \textit{2}. Let $2\leq  p_i< 2^{s_i}$   and $\lambda=(\lambda_1,\lambda_2,\ldots,\lambda_l)$ where $1\leq i\leq l$ and $0\leq\lambda_{i}\leq p_{i}$. Then the set of codes
\begin{equation}
    \begin{split}
 \bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi_{Trun}}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}<p_{i}-1\bigg\}
    \end{split}
\end{equation}
forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$.
\end{theorem}
\begin{IEEEproof}
From (14) and (15) it can be observed that each parenthesis of $\Psi_{Trun}(M^{\mathbf{v},r,d,\lambda,h})$ and $\Psi_{Trun}(N^{\mathbf{v},r,d,\lambda,h})$ can be expressed as  $\omega_{p_1}^{\lambda_1 (i_1)}\omega_{p_2}^{\lambda_2 (i_2)}\ldots\omega_{p_l}^{\lambda_l (i_l)}\Psi(g^{\mathbf{v},\mathbf{r},d,h})$ and  $\omega_{p_1}^{\lambda_1 (i_1)}\omega_{p_2}^{\lambda_2 (i_2)}\ldots\omega_{p_l}^{\lambda_l (i_l)}\Psi(s^{\mathbf{v},\mathbf{r},d,h})$ respectively.
From (11), (14), \textit{Lemma} \textit{2} and \textit{Lemma} \textit{3} the ACCF between $\Psi_{Trun}(\Omega_{r}^{\lambda})$ and ${\Psi_{Trun}}(\Omega_{r'}^{\lambda'})$   for $\tau=0$ can be derived as,\\
~~\\
$~~~\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}}(\Omega_{r'}^{\lambda '}))(0)$\\
~\\
$~~=\displaystyle\sum_{\mathbf{v},d}\Theta({\Psi_{Trun}}(M^{\mathbf{v},\mathbf{r},d,\lambda,h}),{\Psi_{Trun}}(M^{\mathbf{v},\mathbf{r}',d,\lambda',h}))(0)$\\
$~~=\displaystyle\sum_{\mathbf{v},d}\Theta({\Psi}(g^{\mathbf{v},\mathbf{r},d,h}),{\Psi}(g^{\mathbf{v},\mathbf{r}',d,h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}$
\newpage
$=\Theta(\Psi(G_r),\Psi(G_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}$
\begin{equation}
    =\begin{cases}
     p_{1}p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\\
     0         ,& r=r', \lambda\neq\lambda',\\
     0         ,& r\neq r',\lambda=\lambda',\\
     0         ,& r\neq r',\lambda\neq \lambda'.
    \end{cases}~~~~~~~~~~~~~
\end{equation}
Now, Using (11), (14), \textit{Lemma} \textit{2} and  the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ 
and ${\Psi_{Trun}}(\Omega_{t'}^{\lambda^{'}})$ for $0<|\tau|<2^m$ can be derived as,
\begin{equation}
    \begin{split}
        &\Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda^{'}}))(\tau)\\
        &=\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_i-1}\omega_{p_{i}}^{(\lambda_i-\lambda_i^{'})(\alpha)}\\
         &+\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau-2^m)\displaystyle\sum_{\alpha=0}^{p_{1}-2}\omega_{p_{1}}^{\lambda_1(\alpha+1)-\lambda_1^{'}\alpha}\\
        &\prod_{i=2}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_{i}}^{\lambda_i(\alpha)-\lambda_i'(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\displaystyle\sum_{j=1}^{l-2}\prod_{i=1}^{j}\omega_{p_{i}}^{\lambda_{i}(p_{i}-1)-\lambda^{'}_{i}(0)}\displaystyle\sum_{\alpha=0}^{p_{j+1}-2}\omega_{p_{j+1}}^{\lambda_{j+1}(\alpha+1)-\lambda^{'}_{j+1}(\alpha)}\prod_{k=j+2}^{l}\\
        &\displaystyle\sum_{\alpha=0}^{p_{k}-1}\omega_{p_{k}}^{\lambda_{p_{k}}(\alpha)-\lambda^{'}_{p_{k}}(\alpha)}+\Theta(\psi(G_r),\psi(G_{r^{'}}))(\tau-2^m)\\
        &\prod_{i=1}^{l-1}w_{p_i}^{\lambda_i( p_i^{\alpha_i}-1)-\lambda_i^{'}(0)}\displaystyle\sum_{\alpha=0}^{p_{l}^{\alpha_l}-2}\omega_{p_{l}}^{\lambda_{l}(\alpha+1)-\lambda^{'}_{l}\alpha}
    \end{split}
\end{equation}
   From \textit{Lemma} \textit{2} we have
\begin{equation}\label{thpoly7}
\begin{split}
 \Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)=0,~ 0<|\tau|<2^m.
 \end{split}
\end{equation}
From (20) and (21),We have
\begin{equation}
 \begin{split}
    \Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda '}))(\tau)=0,0<|\tau|<2^m.
 \end{split}
\end{equation}
From (19) and (22) We have
\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t'}^{\lambda '}))(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
Similarly, it can be shown that

\begin{equation}\label{thpoly9}
 \begin{split}
  \theta&({\Psi^{*}_{Trun}}(\Lambda_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r'}^{\lambda'})(\tau)\\
  &=\begin{cases}
     p_{1} p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\tau=0,\\
     0         ,& r=r', \lambda\neq\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda=\lambda',0<|\tau|<2^m,\\
     0         ,& r\neq r',\lambda\neq \lambda',0<|\tau|<2^m.
    \end{cases}
 \end{split}
\end{equation}
From \textit{Lemma} \textit{2} we have 
\begin{equation}
     \Theta(\Psi(G_r),\Psi^*(\bar{G}_{r}))(\tau)=0,~ |\tau|<2^m.
\end{equation}
From \textit{Lemma} \textit{2}, (11), (12), (14) and (15) the ACCF between ${\Psi_{Trun}}(\Omega_t^\lambda)$ and ${\Psi_{Trun}^{*}}(\Lambda_{t^{'}}^{\lambda^{'}})$ for $\tau=0$ can be derived as
\begin{equation}
    \begin{split}
    &\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)\\
&=\Theta(\Psi(G_r),\Psi^{*}(\Bar{G}_{r^{'}}))(0)\sum_{\alpha=0}^{p_{1}-1}\omega_{p_1}^{(\lambda_1+\lambda_1^{'})\alpha}\sum_{\alpha=0}^{p_{2}-1}\omega_{p_2}^{(\lambda_2+\lambda_2^{'})\alpha}\\
        &\ldots\sum_{\alpha=0}^{p_{l}-1}\omega_{p_l}^{(\lambda_l+\lambda_l^{'})\alpha}
    \end{split}
\end{equation}
From (25), and (26) we have
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(0)=0
\end{equation}
By the similar calculation as in  (20), we have
\begin{equation}
    \Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}^{*}}(\Lambda_{r^{'}}^{\lambda^{'}})(\tau)=0,\forall~ 0<|\tau|<2^{m}
\end{equation}
Hence by (23), (24), (27) and (28) we  conclude the set
\begin{equation}
\begin{split}
    \Bigg\{{\psi_{Trun}}(\Omega_{r}^{\lambda}),{\psi_{Trun}}^{*}(\Lambda_{r}^{\lambda}):0\leq r<2^{n},&0\leq\lambda_{i}\leq p_{i}-1\Bigg\}
\end{split}
\end{equation}
 forms a $(\prod_{i=1}^{l}p_{i}2^{n+1},2^{m})-ZCCS_{2^{n+1}}^{2^m\prod_{i=1}^{l}p_{i}}$


\end{IEEEproof}


$=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi}(g^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}$




$=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)$
$=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi}(g^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}$\\
&$=\Theta(\Psi(G_r),\Psi(G_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}$




&\Theta({\Psi_{Trun}}(\Omega_r^\lambda),{\Psi_{Trun}}(\Omega_{r'}^{\lambda '}))(0)\\
&=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r},\lambda,h}),{\Psi_{Trun}}(M^{\mathbf{v'},\mathbf{r}',\lambda',h}))(0)\\
&=\displaystyle\sum_{\mathbf{v'}}\Theta({\Psi}(g^{\mathbf{v'},\mathbf{r},h}),{\Psi}(g^{\mathbf{v'},\mathbf{r}',h}))(0)\prod_{i=1}^{l}\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}\\
&=\Theta(\Psi(G_r),\Psi(G_{r'}))(0)\displaystyle\prod_{i=1}^{l}\displaystyle\sum_{\alpha=0}^{p_{i}-1}\omega_{p_i}^{(\lambda_i-\lambda_i')\alpha}\\

    &=\begin{cases}
     p_{1}p_{2}\ldots p_{l}2^{m+n+1},& r=r',\lambda=\lambda',\\
     0         ,& r=r', \lambda\neq\lambda',\\
     0         ,& r\neq r',\lambda=\lambda',\\
     0         ,& r\neq r',\lambda\neq \lambda'.
    \end{cases}
    
    
    
    
    
    From \textit{Lemma} \textit{2} we have

 $\Theta(\Psi(G_r),\Psi(G_{r^{'}}))(\tau)=0,~ 0<|\tau|<2^m.$

Therefore,
\begin{equation}
 \begin{split}
    \Theta({\Psi_{Trun}}(\Omega_t^\lambda),{\Psi_{Trun}}(\Omega_{t^{'}}^{\lambda '}))(\tau)=0,0<|\tau|<2^m.
 \end{split}
\end{equation}






 $ \Psi(M^{\mathbf{v'},\mathbf{r},\lambda,h})=
 &(\omega^{M^{\mathbf{v'},\mathbf{r},\lambda,h}_0}_q, \omega^{M^{\mathbf{v'},\mathbf{r},\lambda,h}_1}_q,\hdots,\omega_q^{M^{\mathbf{v'},\mathbf{r},\lambda,h}_{2^{m+\sum_{i=0}^{l}s_i}-1}})$,
 
 
 
 
 
 $0\leq i_{k}\leq2^{s_k}-1$ , $1\leq k\leq l$ and $0\leq j\leq 2^{m}-1$. Therefore after the trancation we left with a squence $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$  where, each elements of $\Psi_{Trun}(M^{\mathbf{v'},\mathbf{r},\lambda,h})$ is of the form  $w_{q}^{g_{j}^{\mathbf{v'},\mathbf{r},h}}\!w_{p_1}^{\lambda_{1}(i_{1})}\!w_{p_2}^{\lambda_{2}(i_{2})}\!\hdots\!
w_{p_l}^{\lambda_{l}(i_{l})}$\!\! where, $0\!\leq i_{k}\leq\! p_{k}\!-\!1$ , $0\!\leq\! j\!\leq\! 2^{m}\!-\!1$ and $1\leq\! k\!\leq\! l$.






\displaystyle\sum_{k=0}^{s_{i}-1}2^{k}y_{m+{\sum_{j=0}^{i-1}s_{j}+k}}




\omega_q^{{g}^{\mathbf{v'},\mathbf{r},h}(r_0,r_1,\hdots, r_{m-1})}\prod_{i=1}^{l}\omega_{p_{i}}^{\lambda_{i}\displaystyle\sum_{k=0}^{s_{i}-1}2^{k}y_{m+{\sum_{j=0}^{i-1}s_{j}+k}}}




In this work, we have proposed a direct construction of optimal ZCCSs for all possible even lengths using PBFs. The maximum column sequence PMEPR ofthe proposed  ZCCSs is upper-bounded by $2$ which can be useful in MC-CDMA systems to control high PMEPR problem. The proposed construction also provides more flexible parameter as compared to the existing PBFs based construction of optimal ZCCSs.
